Language-Integrated Updatable Views (Extended version)

Relational lenses are a modern approach to the view update problem in relational databases. As introduced by Bohannon et al. (2006), relational lenses allow the definition of updatable views by the composition of lenses performing individual transformations. Horn et al. (2018) provided the first implementation of incremental relational lenses, which demonstrated that relational lenses can be implemented efficiently by propagating changes to the database rather than replacing the entire database state. However, neither approach proposes a concrete language design; consequently, it is unclear how to integrate lenses into a general-purpose programming language, or how to check that lenses satisfy the well-formedness conditions needed for predictable behaviour. In this paper, we propose the first full account of relational lenses in a functional programming language, by extending the Links web programming language. We provide support for higher-order predicates, and provide the first account of typechecking relational lenses which is amenable to implementation. We prove the soundness of our typing rules, and illustrate our approach by implementing a curation interface for a scientific database application.

==> fig/links-db.tex <==
\begin{figure}
    \texttt{albums} \vspace{0.75em}\\
  \begin{tabular}{|c|c|}\hline
    \texttt{album} & \texttt{quantity} \\ \hline
    Disintegration & 6 \\ \hline
    Show & 3 \\ \hline
    Galore & 1 \\ \hline
    Paris & 4 \\ \hline
    Wish & 5 \\ \hline
  \end{tabular}
%
  \vspace{1em} \\
%
  \texttt{tracks}\vspace{0.75em}\\
\begin{tabular}{|c|c|c|c|}\hline
  \texttt{track} & \texttt{year} & \texttt{rating} & \texttt{album} \\ \hline
  Lullaby & 1989 & 3 & Galore \\ \hline
  Lullaby & 1989 & 3 & Show \\ \hline
  Lovesong & 1989 & 5 & Galore  \\ \hline
  Lovesong & 1989 & 5 & Paris \\ \hline
  Trust & 1992 & 4 & Wish \\ \hline
\end{tabular}
  \caption{Music Database}
  \label{fig:music-db-example}
\end{figure}



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../links-lens"
%%% End:


==> fig/mvu.tex <==
\usetikzlibrary{shadows,positioning}
\colorlet{colM}{red!40}
\colorlet{colV}{cyan!40}
\colorlet{colU}{blue!40}
\colorlet{colBorder}{gray!70}
\tikzset
  {mybox/.style=
    {rectangle,rounded corners,drop shadow,minimum height=1cm,
     minimum width=2cm,align=center,fill=#1,draw=colBorder,line width=1pt
    },
   myarrow/.style=
    {draw=#1,line width=3pt,-stealth,rounded corners
    },
   myarrow2/.style=
    {draw=#1,line width=3pt
    },
   mylabel/.style={text=#1}
  }
  \begin{tikzpicture}[font=\sffamily]
  \node[mybox=colM] (M) {Model};
  \node[mybox=colV,right=of M] (V) {View};
  \node[mybox=colU,right=of V] (U) {Update};
  \node[coordinate, below=0.75cm of U] (UC) {};
  \node[coordinate, below=0.75cm of M] (MC) {};
  \draw[myarrow=colV] (M) -- (V);
  \draw[myarrow=colU] (V) -- (U);
  \path (M) -- node[above=1.5em]{\textsf{Render}} (V);
  \path (V) -- node[above=1.5em]{Message} (U);
  \path (UC) -- node[right]{} (MC);
  \draw[myarrow2=colM, midway] (U.south) -- (UC.north);
  \draw[myarrow2=colM, midway,below] (UC.west) -- (MC.east);
  \draw[myarrow=colM, midway] (MC.north) -- (M.south);
\end{tikzpicture}


==> fig/rules_drop_input.tex <==

\[
  \begin{tabular}{|c|c|c|c|}\hline
    \texttt{track} & \texttt{year} & \texttt{rating} & \texttt{album} \\ \hline
    Lovesong & 1989 & 5 & Galore  \\ \hline
    Lovesong & 1989 & 5 & Paris \\ \hline
    Trust & 1992 & 4 & Wish \\ \hline
  \end{tabular}
\]



==> fig/rules_drop_view.tex <==

\[
  \begin{tabular}{|c|c|c|}\hline
    \texttt{track} & \texttt{rating} & \texttt{album} \\ \hline
    Lovesong & \correct{5}{3} & Galore \\ \hline
    Lovesong & \correct{5}{3} & Paris \\ \hline
    Trust & 4 & Wish \\ \hline
  \end{tabular}
\]



==> fig/rules_join_reviews.tex <==

\[
  \begin{tabular}{|c|c|c|}\hline
    \texttt{user} & \texttt{review} & \texttt{album} \\ \hline
    musicfan & 4 & Galore \\ \hline
    90sclassics & 5 & Galore \\ \hline
    thecure & 5 & Paris \\ \hline
  \end{tabular}
\]


==> fig/rules_join_view.tex <==

\[
  \begin{tabular}{|c|c|c|c|c|c|}\hline
    \texttt{user} & \texttt{review} & \texttt{track} & \texttt{year} & \texttt{rating} & \texttt{album} \\ \hline
    musicfan & 4 & Lullaby & 1989 & 3 & Galore \\ \hline
    musicfan & 4 & Lovesong & 1989 & 5 & Galore \\ \hline
    \strikeStart{90sclassics} & 5 & Lullaby & 1989 & 3 & \strikeEnd{Galore} \\ \hline
    90sclassics & 5 & Lovesong & 1989 & 5 & Galore \\ \hline
    thecure & 5 & Lovesong & 1989 & 5 & Paris \\ \hline
  \end{tabular}
\]



==> fig/rules_select_corrected.tex <==

\[
  \begin{tabular}{|c|c|c|c|c|}\hline
    \texttt{track} & \texttt{year} & \texttt{rating} & \texttt{album} &
                                                                        \texttt{quantity} \\ \hline
    Lullaby & 1989 & 3 & Galore & 1 \\ \hline
    Lovesong & 1989 & \correct{5}{4} & Galore  & 1 \\ \hline
    Lovesong & 1989 & \correct{5}{4} & Paris & 4 \\ \hline
    Trust & 1992 & 4 & Wish & 4 \\ \hline
  \end{tabular}
\]


==> fig/rules_select_input.tex <==
\[
  \begin{tabular}{|c|c|c|c|c|}\hline
    \texttt{track} & \texttt{year} & \texttt{rating} & \texttt{album} &
                                                                        \texttt{quantity} \\ \hline
    Lullaby & 1989 & 3 & Galore & 1 \\ \hline
    Lovesong & 1989 & 5 & Galore  & 1 \\ \hline
    Lovesong & 1989 & 5 & Paris & 4 \\ \hline
    Trust & 1992 & 4 & Wish & 4 \\ \hline
  \end{tabular}
\]


==> fig/rules_select_view.tex <==

\[
  \begin{tabular}{|c|c|c|c|c|}\hline
    \texttt{track} & \texttt{year} & \texttt{rating} & \texttt{album} &
                                                                        \texttt{quantity} \\ \hline
    Lullaby & 1989 & 3 & Galore & 1 \\ \hline
    Lovesong & 1989 & \correct{5}{4} & Galore  & 1 \\ \hline
  \end{tabular}
\]


